"We Have No Idea How Models will Behave in Production until Production": How Engineers Operationalize Machine Learning

Organizations rely on machine learning engineers (MLEs) to deploy models and maintain ML pipelines in production. Due to models' extensive reliance on fresh data, the operationalization of machine learning, or MLOps, requires MLEs to have proficiency in data science and engineering. When considered holistically, the job seems staggering -- how do MLEs do MLOps, and what are their unaddressed challenges? To address these questions, we conducted semi-structured ethnographic interviews with 18 MLEs working on various applications, including chatbots, autonomous vehicles, and finance. We find that MLEs engage in a workflow of (i) data preparation, (ii) experimentation, (iii) evaluation throughout a multi-staged deployment, and (iv) continual monitoring and response. Throughout this workflow, MLEs collaborate extensively with data scientists, product stakeholders, and one another, supplementing routine verbal exchanges with communication tools ranging from Slack to organization-wide ticketing and reporting systems. We introduce the 3Vs of MLOps: velocity, visibility, and versioning -- three virtues of successful ML deployments that MLEs learn to balance and grow as they mature. Finally, we discuss design implications and opportunities for future work.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
# See main.pdf

This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/reviewer_response.tex <==
\newcommand{\wuu}[1]{\subsection*{#1}}
\newcommand{\com}[1]{\smallskip \noindent \textcolor{purple}{{\em #1}}}
\newcommand{\ans}[1]{\vspace{12pt}\noindent #1}



\section*{Summary for Revised Paper\\{\em``We have no idea how models will behave in production until production''}: How engineers operationalize machine learning}

We thank the reviewers and meta-reviewer 
for their insightful, detailed feedback and for giving us the opportunity to
address the issues in a major revision. Over the last 6 months, we have iterated several times on the interview transcripts and paper manuscript to improve the exposition and motivation of the paper, related work, methods, and presentation of findings.
The prominent changes include:

\smallskip
\noindent {\em {\bf A. A rewritten description of our methods.}} In response to feedback regarding the clarity of our methodology, and to answer questions about the scope of our findings, we have made substantial revisions to our methods section (\Cref{sec:methods}). This revised section now prominently describes our use of grounded theory for our findings. We elaborate on our iterative data collection and analysis process, emphasizing the constant comparative method and our approach for reaching theoretical saturation. We have added an abridged code system  (\Cref{fig:codebook}), and significantly expanded the table of participants (\Cref{tab:interviewees}). By clarifying our methodology, we aim to offer readers a more transparent and comprehensive understanding of our research approach.

\smallskip
\noindent  {\bf B. Additional related work.} We have a new section dedicated to a review of the recent MLOps literature  (\Cref{sec:related-mlops}). In this section, we discuss how prior work demonstrates a gap in the community's understanding of human-centered processes in MLOps. Our paper interviews ML engineers to characterize such processes, as well as common challenges ML engineers face.

\smallskip
\noindent  {\bf C. An improved presentation of results.} We have revised our summary of findings, repositioning our results with the MLOps literature as well as data science-related work from the CHI and CSCW communities. Additionally, we have included a comprehensive table of human-centered processes and challenges uncovered in our interviews (\Cref{app:interviewq}),

% \noindent\textbf{\textit{A complete rewrite of the introduction to~\Cref{sec:methods} (Methods), with evidence for theoretical saturation}.}

% \rolando{TODO}


% \noindent\textbf{\textit{A new~\Cref{sec:related-mlops} (Related Work) with thorough coverage of the MLOps literature}.}

% Aligned with the feedback from Reviewer \#1, we have written a new section dedicated to a review of the MLOps literature. This section situates our work within the existing academic landscape: while many papers have identified MLOps challenges by surveying tools and investigating the \emph{automated} practices of the MLOps lifecycle, there is an opportunity to investigate the \emph{human-centered} workflow of ML engineers, or people responsible for ML models in production. Our work conducts the first semi-structured study focused solely on ML engineers, with the intent of discovering common themes in their workflows and pain points across different organizational maturity levels and industries. 

% \noindent\textbf{\textit{An improved presentation of results across~\Cref{sec:summary,sec:discussion}, including a summary table of findings and a detailed table of tools referenced by interviewees.}}

% Acknowledging the feedback from Reviewers \#2 and \#3, we have improved the presentation of our results. In addition to positioning specific findings with the MLOps literature, this revision includes a summary table of findings to provide a succinct overview of the key challenges experienced by the interviewees. Furthermore, we have introduced a detailed table in~\Cref{app:tools} cataloging the various systems and tools referenced by the interviewees, as per Reviewer \#3's suggestion.


\smallskip
\noindent The changes in the paper are highlighted in \textcolor{blue}{\textbf{blue}}. We begin by addressing each point raised in the metareview.

\ \\[-0.75em]\noindent{\bf Metareview}

\com{(MR1) Reviewer \#1 raises questions about the external validity of the study due to the limited number of interviewees (18) and requests evidence of theoretical saturation. This aligns with Reviewer \#2's request for a clearer presentation of the participant selection process. Although Table 1 offers some background on the interviewees, the paper doesn't discuss it in detail. Critical inquiries, such as the interviewees' years of experience in ML and MLOps, their educational background, and the development culture of their companies, are not currently addressed but might offer deeper insights into the sample.
}

We agree that the original submission was lacking a rich description of how we reached theoretical saturation in our interviews. We have rewritten the introduction of our methods section (\Cref{sec:methods}) to discuss how we alternated between interviews and data analysis---each round of interviews was followed by in-depth coding of transcripts. We deemed our interview process complete when subsequent interviews did not yield new themes. Altogether, we engaged in 6 rounds of interviews, or 18 total interviews. We note that in qualitative research, theoretical saturation is often reached within a range of 12 to 30 participants, especially in homogeneous populations~\cite{guest2006many}. Additionally, recruitment of participants in highly specialized domains, such as ML Engineers in our case, is challenging. Prior work employing
semi-structured interview studies with participants from related domains, such as data scientists, typically have between 10--20 participants (e.g., 10~\cite{kross2019practitioners}, 16~\cite{whitherautoml}, 20~\cite{autoai}, as we do.

In line with Reviewer \#2's suggestion, we have added many more columns to our table of interviewees (\Cref{tab:interviewees}); including the size of their company, application area (i.e., industry), years of experience with ML engineering, geographic location, and most prominent codes from their interview transcripts---which provides insights on the culture and priorities of their organization. We intentionally picked our interviewees to span a diversity of experiences, applications, and demographics with the goal of determining common patterns.

Finally, in our revision, we have added~\Cref{fig:codebook}, an abridged version of our codebook, to demonstrate the results of using grounded theory to analyze our findings. We believe this will shed additional light on how our findings were derived from the interviews. For each of the human-centered processes uncovered by our codes, we situate them among the automated processes in the machine learning lifecycle.

\com{(MR2) Reviewer \#1 also points out that the paper should more carefully position
itself with respect to the state of the art. According to the Reviewer, the paper
does not provide an overall perspective over current works in MLOps.}

After reflecting on the related work in our original submission, we agree that some recent related works in MLOps were missing. In our revision, we add an entirely new section (\Cref{sec:related-mlops}) dedicated to the MLOps literature, including all of the pointers Reviewer \#1 shared, as well as others we could find---particularly from 2022. Additionally, in the summary of findings and discussion sections (\Cref{sec:summary,sec:discussion}), wherever relevant, we have compared and contrasted our results to findings from the recent MLOps literature.

In our revision, we note that there is little consensus on what an ML lifecycle entails among the related work, indicating that the field is still in its nascency. We survey papers describing case studies of organizations describing good MLOps hygiene within their teams, vision papers of what MLOps should entail, and tool surveys to uncover automated processes in the ML lifecycle. What's missing in the related work is the understanding of the human-centered processes and pain points when productionizing ML, motivating our research. While some of the related work has interviewed some people involved in building automated parts of the production ML lifecycle~\cite{mlopsoda}, such as data engineers, to the best of our knowledge, our paper is the first to solely interview ML engineers, with the goal of identifying the manual processes and pain points in their workflows. Our findings demonstrate that there are considerable challenges ML engineers face when automating ML pipelines, from sifting through thousands of automated data quality alerts to continuously testing pipelines on dynamic datasets.


\com{(MR3) Reviewer \#2 reports that the presentation of the results might be improved,
for instance by discussing the differences obtained when considering interviewees
working in large and small companies (if any). Still in terms of results, Reviewer
\#3 suggests to specify or reference some of the systems and tools cited in the
paper, perhaps in an online appendix that readers might want to consult.}

We appreciate the constructive feedback regarding the presentation of our results. First, to address Reviewer \#2's feedback, we have introduced a comprehensive table summarizing the human-centered processes and challenges identified during our study (\Cref{tab:summaryfindings}). We believe this new table serves as a roadmap for the summary of findings and discussion sections (\Cref{sec:summary,sec:discussion}), enhancing the readabilty of our results. Second, with regards to Reviewer \#3’s advice, we have catalogued the systems and tools referenced by our interviewees and segmented them by stage in the MLOps workflow. This detailed table has been included in the appendix of our paper (\Cref{app:tools}). 

Finally, we acknowledge Reviewer \#2's suggestion to discuss differences in responses between interviewees from large and small companies. However, the primary goal of our study was to identify common themes and practices amongst ML engineers, irrespective of their company size, emphasizing universal experiences over company-specific variations. As such, we have added a subsection in the Limitations and Future Work section (\Cref{sec:discussion-limitations}) to clarify our rationale. We note that there are further opportunities, possibly in future work, to study the effect of organizational maturity on production ML workflows. Nonetheless, to indicate potential trends or discrepancies observed across different company sizes without distracting from our focus on common themes, we reference participants in our revision by company size (e.g., Sm1 or Sm2 instead of P1 or P2). 

\ \\[-0.75em]\noindent{\bf Reviewer 1}

\com{(W1) From the related work standpoint, the authors largely neglect to provide an overview of current MLOps research. Despite the growing number of both early-stage and mature findings in the areas of MLOps reference architectures, sustainability, and the role of the MLOps engineer, these topics are not adequately covered.}

We thank the reviewer for their feedback and add a new section (\Cref{sec:related-mlops}) to cover current works in MLOps, including the ones referenced by the reviewer. While current work covers several pain points, case studies, and reference architectures for automated processes in MLOps, we note an opportunity to study the human-centered processes that ML engineers engage in by interviewing them directly. As discussed in our response for M2 above, to the best of our knowledge, a semi-structured interview study solely focused on ML engineers fills a gap in the research literature that has not prioritized their needs, workflows, or challenges. Our work uncovers new insights and opportunities for tooling, as discussed in~\Cref{sec:summary,sec:discussion}.

\com{(W2) From a generalizability standpoint, the study's external validity is questionable due to the limited (18) interviews conducted. While the number of interviews might be adequate, there's no presented evidence to support this sufficiency. It's unclear if the dataset has been tested for theoretical saturation.}

We are grateful for the reviewers' constructive feedback on our sample size's generalizability. In response, we have carefully revised the introduction to the methods section to better articulate our objectives and context, as detailed in \Cref{sec:methods}. While our number of interviews may initially appear limited, our targeted sample size allowed for iterative, in-depth examinations of each interview. This iterative approach persisted until we observed a saturation of new insights, which was notably evident by our 16th interview where consistent patterns solidified (\cref{tab:interviewees}). This sample size is consistent with qualitative research norms, such as the findings of \citet{guest2006many}, suggesting that saturation typically emerges between 12 to 30 interviews, especially when participants possess overlapping characteristics.

\com{(W3) * minor comments *
- intro, line 31: "Why MLOps is hard" - is -> ARE;
- line 34: why are "technical debt" and "massive ongoing..." in quotes? please
provide a definition and references;
- intro, past paragraph: add the structure of the article;}

We thank the reviewer for finding these issues. We have addressed the typos and added an outline in the introduction. We note that the original submission had the reference related to technical debt (i.e., \citet{Sculley2015HiddenTD}), and the phrases in quotes were in quotes because they were taken directly from the paper. We have reworded this sentence in the revision to eliminate any source of confusion.

\ \\[-0.75em]\noindent{\bf Reviewer 2}

\com{(W1) The process conducted to select participants should be better detailed in the
article.}

See our response to (MR1) above and (D3) and (D4) below.

\com{(W2) The presentation of the results could be improved.}

See our response to (MR2) above and (D5) below.

\com{(D1) Related work: While the analysis of the state of the art conducted give a lot of articles that
proposes different stage in ml workflow, I suggest considering these two points:
First, include also CRISP-DM and CRISP-ML (Q)
Second, (see in discussion), discuss the merge of evaluation and deployment stage.}

We thank the reviewer for these comments. Addressing the first point, we have included the CRISP-DM and CRISP-ML (Q) references in \Cref{sec:related}. Addressing the second point, we have revised~\Cref{sec:summary-eval} to clearly articulate why we merged the evaluation and deployment stages. We combine these stages because they are tightly intertwined, with deployments spanning long periods of time and evaluations happening repeatedly and periodically throughout the deployment. 

\com{(D2) Related work: It would be interesting to add information about tools that
supports the entire pipeline of Machine learning: (e.g, MLFlow).
Different studies are conducted on the feature and tools proposed for MLOps.}

We thank the reviewer for the references provided and have incorporated them into the new~\Cref{sec:related-mlops} in the revision, motivating the study of how engineers such tools. We did another pass on our interview transcripts to categorize tools mentioned across stages of our MLOps workflow, and we have added a table of tools in~\Cref{app:tools}.



\com{(D3, D4) Participant Recruitment involves examining various factors such as educational backgrounds, years of experience, roles, team size, and the sector of work. The key question raised is whether this data is beneficial for selecting appropriate candidates. Furthermore, clarity is sought on any criteria used to determine the eligibility of interview participants. In the methodology section, a more extensive description of the qualitative analysis applied is needed. While the Straussian Grounded Theory details techniques for the first and second cycle of analysis, more information on the application of these techniques is requested. It's also vital to continuously consider the backgrounds of the participants. The uniqueness or significant differences in the participant set, based on their backgrounds, should be analyzed further. A recommendation has been made to modify Table 1 to delve deeper into the backgrounds of the participants. For instance, how does working for a large company versus a small one impact the challenges identified by different participants?
}

In light of the feedback received, we've reworked the presentation of our methodology, focusing on our approach to participant recruitment and the scope of our application of grounded theory. The reviewers' insights underscored the importance of detailing demographics and ensuring a thorough qualitative analysis. Below, we describe our refined approach and address each highlighted area.

\begin{enumerate}
\item We expanded our participant table to capture demographic shifts across different rounds (\Cref{tab:interviewees}), as it illustrates our iterative, theoretical sampling approach. For instance, initially, on the first round (RR=1) our sample had fewer participants from small companies. In the subsequent round, we intentionally targeted smaller companies to achieve balance.
\item Participant Eligibility and Selection: Our eligibility criteria for participants primarily focused on their role as ML engineers and their experience in the field. We sought diversity in educational backgrounds, years of experience, team sizes, and work sectors to capture a broad spectrum of perspectives. Our recruitment process involved outreach through academic and industry networks, and participants were selected based on their relevance to the study and their availability.
\item Reflexivity and Context: Recognizing the importance of reflexivity in qualitative research, we've added a paragraph giving some context on ourselves --- as the instruments of observation, our motivations for this study, and why we deeply care about the subject matter (\Cref{sec:methods}). We believe this detail adds another layer of transparency to our methods and helps readers understand the context from which our inquiries originated.
\item Detailed Application of Grounded Theory: Our qualitative analysis started with open coding where we identified initial concepts from the interview data. This was followed by axial coding, where these concepts were categorized into themes. During selective coding, we refined these themes, ensuring they were grounded in the data, and integrated them into our theoretical framework. Throughout this process, memos and annotations were made to track our thought process and the development of the theory. The outcome of this iterative process is presented in our abridged code book, which has been added to the revised manuscript (\Cref{fig:codebook}).
\end{enumerate}



\com{(D5) While the results are well discussed, it could be better to restructure the
section to increase the readability. In detail, I suggest to:
Create an “Overview section” in which a mapping between the issues and challenges
highlighted by the participants and the areas of ML involved should be presented.
Restructure the other sections based on the research question that should be
answered. Add tables or plots that directly shows the list of challenges identified for
areas.}

Acknowledging this feedback, our revision includes a table covering human-centered practices and pain points for each stage in the MLOps workflow (\Cref{tab:summaryfindings}). This overview table is presented in the beginning of our findings (\Cref{sec:summary}), to improve the overall presentation and structure each of our findings. For more details, see our response to (MR3) above.

\com{(D6) Figure 1: It could be more relative to the topic to consider a MLOps defined
workflow instead of a general data science workflow.}

This is an interesting idea, which we strongly considered incorporating into our revision. However, in~\Cref{fig:tasksdiagram}, we ultimately decided to compare our MLOps workflow to the workflow prescribed by~\citet{autoai} for a couple of reasons. First, there is no single or predominant MLOps workflow established by prior work, which we discuss further in~\Cref{sec:related-mlops}.~\citet{autoai} has been widely cited (250+ citations). Second, the workflow prescribed by~\citet{autoai} was derived from an interview study of data science practitioners focused on human-centered activities and opinions around AutoAI tools, or systems that intend to automate data science workflows. We find this theme to be relevant to our work, which aims to uncover human-centered practices and challenges in the context of automated, end-to-end production ML pipelines.

\com{(D7) Various typos.}

We thank the reviewer for pointing out these typos, which we have fixed in the revision.

\ \\[-0.75em]\noindent{\bf Reviewer 3}

\com{(W1) The semi-structured interviews were well-executed and grasped the work practices
of participants. The quotes illustrate the author's points and offer reflections
for the readers. Data analysis was well executed; the authors proposed a chart
showing how the data was codified according to the themes during the execution of
the inspired Grounded theory approach. This chart gave the transparency of the
analysis straightforwardly and understandably. More details of participants are
needed to bring the strength of evidence and validation of the issues raised.}

We thank the reviewer for their kind and encouraging feedback. In our revision, we include more details of participants in \Cref{tab:interviewees}, including years of experience, location, organization size, application, and most prominent codes from their transcripts. The revision also includes more evidence for theoretical saturation---see our response to (MR1).

\com{(W2) It might be relevant to specify or reference some of the systems and tools (5.2)
cited in the paper. Maybe a link that readers can consult to know what it is.}

We agree that such a table would not only be relevant, but particularly valuable to people interested in building tools for ML engineers. As such, our revision includes a detailed table of systems and tools used by the participants, categorized by stage in the MLOps workflow. This table can be found in \Cref{app:tools}.
